A Modular Conditional Diffusion Framework for Image Reconstruction

Diffusion Probabilistic Models (DPMs) have been recently utilized to deal with various blind image restoration (IR) tasks, where they have demonstrated outstanding performance in terms of perceptual quality. However, the task-specific nature of existing solutions and the excessive computational costs related to their training, make such models impractical and challenging to use for different IR tasks than those that were initially trained for. This hinders their wider adoption, especially by those who lack access to powerful computational resources and vast amount of training data. In this work we aim to address the above issues and enable the successful adoption of DPMs in practical IR-related applications. Towards this goal, we propose a modular diffusion probabilistic IR framework (DP-IR), which allows us to combine the performance benefits of existing pre-trained state-of-the-art IR networks and generative DPMs, while it requires only the additional training of a relatively small module (0.7M params) related to the particular IR task of interest. Moreover, the architecture of the proposed framework allows for a sampling strategy that leads to at least four times reduction of neural function evaluations without suffering any performance loss, while it can also be combined with existing acceleration techniques such as DDIM. We evaluate our model on four benchmarks for the tasks of burst JDD-SR, dynamic scene deblurring, and super-resolution. Our method outperforms existing approaches in terms of perceptual quality while it retains a competitive performance with respect to fidelity metrics.

==> camera_ready/images/burstsr_synth.tex <==
\begin{figure*}[t]
\centering
\setlength\extrarowheight{-10pt}
\begin{tabular}{@{\hskip 0.05cm} c @{\hskip 0.05cm} c @{\hskip 0.05cm} c @{\hskip 0.05cm} c @{\hskip 0.05cm} c @{\hskip 0.05cm}}
  \multirow{3}{*}[2.31cm]{\includegraphics[width=.29\linewidth]{figures/burst_sr/targets_box/0190_target.png}} &
 \includegraphics[width=.170\linewidth]{figures/burst_sr/0190_DBSR_201x205_140x180.png} & 
 \includegraphics[width=.170\linewidth]{figures/burst_sr/0190_DeepRep_201x205_140x180.png} & 
 \includegraphics[width=.170\linewidth]{figures/burst_sr/0190_BSRT_S_201x205_140x180.png} &
 \includegraphics[width=.170\linewidth]{figures/burst_sr/0190_BSRT_L_201x205_140x180.png} \\
 & \cts{DBSR} & \cts{DeepRep} & \cts{BSRT-Small} & \cts{BSRT-Large} \\
 
 & \includegraphics[width=.170\linewidth]{figures/burst_sr/0190_target_201x205_140x180.png} & 
 \includegraphics[width=.170\linewidth]{figures/burst_sr/0190_BIPNet_201x205_140x180.png} & 
 \includegraphics[width=.170\linewidth]{figures/burst_sr/0190_EBSR_201x205_140x180.png} &
 \includegraphics[width=.170\linewidth]{figures/burst_sr/0190_SDM_25_201x205_140x180.png} \\
  & \cts{Target} & \cts{BIPNet} & \cts{EBSR} & \cts{Ours}
\end{tabular}
   \caption{ABC.}
\label{fig:burst_images}
\end{figure*}


\begin{figure*}[t]
\centering
\setlength\extrarowheight{-10pt}
\begin{tabular}{@{\hskip 0.05cm} c @{\hskip 0.05cm} c @{\hskip 0.05cm} c @{\hskip 0.05cm} c @{\hskip 0.05cm} c @{\hskip 0.05cm}}
  \multirow{3}{*}[2.31cm]{\includegraphics[width=.29\linewidth]{figures/burst_sr/targets_box/0209_target.png}} &
 \includegraphics[width=.170\linewidth]{figures/burst_sr/0209_DBSR_0x212_140x180.png} & 
 \includegraphics[width=.170\linewidth]{figures/burst_sr/0209_DeepRep_0x212_140x180.png} & 
 \includegraphics[width=.170\linewidth]{figures/burst_sr/0209_BSRT_S_0x212_140x180.png} &
 \includegraphics[width=.170\linewidth]{figures/burst_sr/0209_BSRT_L_0x212_140x180.png} \\
 & \cts{DBSR} & \cts{DeepRep} & \cts{BSRT-Small} & \cts{BSRT-Large} \\
 
 & \includegraphics[width=.170\linewidth]{figures/burst_sr/0209_target_0x212_140x180.png} & 
 \includegraphics[width=.170\linewidth]{figures/burst_sr/0209_BIPNet_0x212_140x180.png} & 
 \includegraphics[width=.170\linewidth]{figures/burst_sr/0209_EBSR_0x212_140x180.png} &
 \includegraphics[width=.170\linewidth]{figures/burst_sr/0209_SDM_25_0x212_140x180.png} \\
  & \cts{Target} & \cts{BIPNet} & \cts{EBSR} & \cts{Ours}
\end{tabular}
   \caption{ABC.}
\label{fig:burst_images}
\end{figure*}

\begin{figure*}[t!]
\centering
\setlength\extrarowheight{-10pt}
\begin{tabular}{@{\hskip 0.05cm} c @{\hskip 0.05cm} c @{\hskip 0.05cm} c @{\hskip 0.05cm} c @{\hskip 0.05cm} c @{\hskip 0.05cm}}
  \multirow{3}{*}[2.31cm]{\includegraphics[width=.29\linewidth]{figures/burst_sr/targets_box/0176_target.png}} &
 \includegraphics[width=.170\linewidth]{figures/burst_sr/0176_DBSR_0x104_70x90.png} & 
 \includegraphics[width=.170\linewidth]{figures/burst_sr/0176_DeepRep_0x104_70x90.png} & 
 \includegraphics[width=.170\linewidth]{figures/burst_sr/0176_BSRT_S_0x104_70x90.png} &
 \includegraphics[width=.170\linewidth]{figures/burst_sr/0176_BSRT_L_0x104_70x90.png} \\
 & \cts{DBSR} & \cts{DeepRep} & \cts{BSRT-Small} & \cts{BSRT-Large} \\
 
 & \includegraphics[width=.170\linewidth]{figures/burst_sr/0176_target_0x104_70x90.png} & 
 \includegraphics[width=.170\linewidth]{figures/burst_sr/0176_BIPNet_0x104_70x90.png} & 
 \includegraphics[width=.170\linewidth]{figures/burst_sr/0176_EBSR_0x104_70x90.png} &
 \includegraphics[width=.170\linewidth]{figures/burst_sr/0176_SDM_25_0x104_70x90.png} \\
  & \cts{Target} & \cts{BIPNet} & \cts{EBSR} & \cts{Ours}
\end{tabular}
   \caption{Visual comparison of our approach against competing methods on the Burst JDD-SR task (best viewed by zooming in).}
   
\label{fig:burst_images}
\end{figure*}



==> camera_ready/results/table_ablation_fuser.tex <==

\begin{table}[t]
\caption{Ablation on various fusion networks on DIV2K validation for $4\times$ SR task}
\tts
\centering
\tabcolsep=0.23cm
\label{table:ablation_fuser}
\begin{tabular}{l|ccc|c}
\hline 
Fusion Module                    & PSNR$\uparrow$ & SSIM$\uparrow$  & LPIPS$\downarrow$ & Params \\ \hline
TDWA                             & 27.26          & 0.751           & 0.266             & 8385   \\ 
L-DWT                            & 29.27	      & 0.818 	        & 0.233             & 30.0M  \\
U-Net                            & 28.19          & 0.785           & 0.141             & 31.0M  \\ 
Proposed Fusion                  & 27.93          & 0.777           & 0.149             & 0.7M   \\ \hline
\end{tabular}
\end{table}


==> camera_ready/results/table_ablation_pp.tex <==
\begin{table}[t]
\caption{Ablation on various denoiser and IR networks on DIV2K validation for $4\times$ SISR.}
\small
\centering
\tabcolsep=0.1cm
\label{table:ablation_plug_play}
\begin{tabular}{ll|cc|cc}
\hline 
Denoiser & IR Network    & PSNR\tts{$\uparrow$} & SSIM\tts{$\uparrow$}  & LPIPS\tts{$\downarrow$} & TOPIQ\tts{$\uparrow$} \\ \hline
UDP                              & RRDB   & 27.93          & 0.777        & 0.149        & 5.481        \\ 
MIRNet-S                         & RRDB   & 28.12          & 0.795        & 0.150        & 5.473        \\ 
MIRNet-S                         & SwinIR & 28.12          & 0.793        & 0.140        & 5.485        \\ \hline
\end{tabular}
\end{table}


==> camera_ready/results/table_ablation_tau.tex <==
\begin{table}[!t]
\centering
\caption{Perception-Distortion Trade-off on DIV2K validation for $4\times$ SISR. The \glb{best} values for the metric are highlighted.}
\tts
\centering
\tabcolsep=0.09cm
\label{table:ablation_tau}
\begin{tabular}{l|ccccccc}
\hline
Timestep, $\tau$   & 50          & 100   & 150   & 200   & 250    & 300    & 350         \\ \hline
PSNR $\uparrow$    & \glb{28.77} & 28.46 & 28.24 & 28.06 & 27.93  & 27.81  & 27.71       \\
LPIPS$\downarrow$  & 0.170       & 0.161 & 0.155 & 0.152 & 0.149  & 0.147  & \glb{0.146} \\ \hline 
\end{tabular}
\end{table}



==> camera_ready/results/table_burst.tex <==
\begin{table}[t]
\caption{Performance evaluation on Burst JDD-SR. We highlight the overall \glb{best} for each metric.}  
\tts
\centering
\tabcolsep=0.05cm
\label{table:burst_results}
\begin{tabular}{l|cc|cc|cc}
\hline
Methods    & PSNR\tts{$\uparrow$} & SSIM\tts{$\uparrow$}  & LPIPS\tts{$\downarrow$} & TOPIQ$_{\Delta}$\tts{$\downarrow$} & NFE \tts{$\downarrow$} & Params\tts{$\downarrow$} \\ \hline
Target            & $\infty$    & 1           & 0            & 0           & N/A  & N/A   \\ \hline
DBSR              & 31.98       & 0.891       & 0.198        & 0.10        & N/A  & 13.0M \\
DeepRep           & 34.66       & 0.927       & 0.136        & 0.07        & N/A  & 12.1M \\
EBSR              & 36.05       & 0.940       & 0.111        & 0.15        & N/A  & 26.0M \\
BIPNet            & 34.86       & 0.934       & 0.112        & 0.03        & N/A  & 6.7M  \\
BSRT-Small        & 35.91       & 0.940       & 0.109        & 0.12        & N/A  & 4.9M  \\
BSRT-Large        & \glb{36.98} & \glb{0.947} & 0.095        & 0.16	       & N/A  & 20.7M \\ \hline
Ours              & 35.53       & 0.933       & \glb{0.084}  & \glb{0.02}  & 6    & 21.6M \\ \hline
\end{tabular}
\end{table}


==> camera_ready/results/table_deblurring_gopro.tex <==
% -============================================> GOPRO GOPRO 
\begin{table}[t]
\caption{Performance evaluation on the GoPro test set for dynamic scene deblurring. $^\dagger$ indicates that a public implementation is unavailable and the metrics are copied from the authors' paper. We highlight the overall \glb{best} for each metric, and the \lcl{best} among perceptual-oriented methods.}
\tts
\centering
\tabcolsep=0.05cm
\label{table:gopro_results}
\begin{tabular}{l|cc|cc|cc}
\hline
Methods    & PSNR\tts{$\uparrow$} & SSIM\tts{$\uparrow$}  & LPIPS\tts{$\downarrow$} & TOPIQ\tts{$\uparrow$} & NFE \tts{$\downarrow$} & Params\tts{$\downarrow$} \\ \hline
Target              & $\infty$    & 1           & 0            & 4.061        & N/A  & N/A \\ \hline
HINet               & 32.77       & 0.960       & 0.088        & 4.028        & N/A  & 88.6M \\
MPRNet              & 32.66       & 0.959       & 0.089        & 4.034        & N/A  & 20.1M \\
MIMO-UNet+          & 32.44       & 0.957       & 0.091        & 4.027        & N/A  & 16.1M \\
NAFNet              & 33.71       & 0.967       & 0.078        & 4.044        & N/A  & 67.9M \\
Restormer           & 32.90       & 0.961       & 0.084        & 4.043        & N/A  & 26.1M \\
FFTFormer           & \glb{34.21} & \glb{0.969} & 0.071        & 4.049        & N/A  & 16.6M \\ \hline
\multicolumn{7}{c}{Perceptual-oriented Methods}                                             \\ \hline
DeblurGANv2         & 29.08       & 0.918       & 0.117        & 4.036        & N/A  & 60.9M \\
DvSR$^\dagger$      & 31.66       & 0.948       & 0.059        & -            & 500  & 26.1M \\
icDPM$^\dagger$     & 31.19       & 0.943       & 0.057        & -            & 500    & 52.0M \\
InDi$^\dagger$      & 31.49       & 0.946       & 0.058        & -            & 10   & 27.7M \\
Ours                & \lcl{33.72} & \lcl{0.963} & \glb{0.053}  & \glb{4.050}  & 6    & 33.2M \\ \hline
\end{tabular}
\end{table}


==> camera_ready/results/table_super_res.tex <==
\begin{table}[!t]
\caption{Performance evaluation on the DIV2K validation set for $4\times$ SISR. We highlight the overall \glb{best} for each metric, and the \lcl{best} among perceptual-oriented methods.}
\tts
\centering
\tabcolsep=0.03cm
\label{table:div2k_results}
\begin{tabular}{l|cc|cc|cc}
\hline 
Methods    & PSNR\tts{$\uparrow$} & SSIM\tts{$\uparrow$}  & LPIPS\tts{$\downarrow$} & TOPIQ\tts{$\uparrow$} & NFE \tts{$\downarrow$} & Params\tts{$\downarrow$} \\ \hline
Target       & $\infty$       & 1.000        & 0.000        & 5.487        & N/A   & N/A \\ \hline
SRResNet     & 29.07          & 0.824        & 0.266        & 5.441        & N/A   & 1.5M \\
RRDB         & 29.48          & 0.834        & 0.254        & 5.449        & N/A   & 16.7M \\
SwinIR       & 29.63          & 0.837        & 0.248        & 5.457        & N/A   & 11.9M \\
LIIF         & 29.30          & 0.830        & 0.258        & 5.441        & N/A   & 22.3M \\
HAT          & \glb{29.75}    & \glb{0.840}  & 0.245        & 5.452        & N/A   & 20.6M \\ \hline
\multicolumn{7}{c}{Perceptual-oriented Methods} \\ \hline
ESRGAN       & 26.64           & 0.758        & \glb{0.115} & 5.501        & N/A   & 16.7M \\
HCFlow       & 27.02          & 0.766        & 0.124        & 5.466        & N/A   & 23.2M \\ 
SwinIR-GAN   & 24.88          & 0.734        & 0.222        & 5.602        & N/A   & 11.9M \\ 
LDM          & 23.30          & 0.697        & 0.218        & 5.506        & 100   & 169.0M \\
SRDiff       & 27.14          & 0.773        & 0.129        & 5.479        & 100   & 23.6M \\
InDI         & 26.45          & 0.741        & 0.136        & 5.478        & 100   & 62.3M \\   
IDM          & 27.35          & 0.782        & 0.147        & 5.479        & 2000  & 116.6M \\
Ours         & \lcl{28.12}    & \lcl{0.793}  & 0.140        & \glb{5.485}  & 51    & 28.5M \\ \hline
\end{tabular}
\end{table}


